RustEvo^2: An Evolving Benchmark for API Evolution in LLM-based Rust Code Generation

Large Language Models (LLMs) have become pivotal tools for automating code generation in software development. However, these models face significant challenges in producing version-aware code for rapidly evolving languages like Rust, where frequent Application Programming Interfaces (API) changes across versions lead to compatibility issues and correctness errors. Existing benchmarks lack systematic evaluation of how models navigate API transitions, relying on labor-intensive manual curation and offering limited version-specific insights. To address this gap, we present RustEvo, a novel framework for constructing dynamic benchmarks that evaluate the ability of LLMs to adapt to evolving Rust APIs. RustEvo automates dataset creation by synthesizing 588 API changes (380 from Rust standard libraries, 208 from 15 third-party crates) into programming tasks mirroring real-world challenges. These tasks cover four API evolution categories: Stabilizations, Signature Changes, Behavioral Changes, and Deprecations, reflecting their actual distribution in the Rust ecosystem. Experiments on state-of-the-art (SOTA) LLMs reveal significant performance variations: models achieve a 65.8% average success rate on stabilized APIs but only 38.0% on behavioral changes, highlighting difficulties in detecting semantic shifts without signature alterations. Knowledge cutoff dates strongly influence performance, with models scoring 56.1% on before-cutoff APIs versus 32.5% on after-cutoff tasks. Retrieval-Augmented Generation (RAG) mitigates this gap, improving success rates by 13.5% on average for APIs released after model training. Our findings underscore the necessity of our evolution-aware benchmarks to advance the adaptability of LLMs in fast-paced software ecosystems. The framework and the benchmarks are publicly released at https://github.com/SYSUSELab/RustEvo.

==> sections/X_move_to_2_MotivationExample.tex <==
\section{Motivation Example}
\label{sec:motivation}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/2_Motivation/motivation.pdf}
    \caption{Motivation Example}
    \label{fig:motivation}
\end{figure}

To illustrate the challenges of code generation in the context of evolving APIs, we consider a real-world case from the Rust ecosystem. In Rust 1.77.0 (released in March 2024), the \texttt{slice::first\_chunk\_mut} method\footnote{XXX} was stabilized, providing a safer and more efficient way to obtain a reference to the first N elements of a slice as a fixed-size array.  
Figure \ref{fig:motivation} presents a programming task that implicitly requires using an API that was stabilized well before the model’s knowledge cutoff date. However, when prompted with this task, \claude~\cite{anthropic2024claude3}—a state-of-the-art (SOTA) LLM with a knowledge cutoff in April 2024—still generates code relying on an older, less safe pattern involving unsafe pointer casting and manual length checking. While this approach remains functional, it introduces unnecessary unsafe code and forgoes the benefits of improved safety and readability. In contrast, when explicitly informed about the API evolution, the same model correctly utilizes \texttt{slice::first\_chunk\_mut}, producing more concise and robust code.  

This example highlights a fundamental challenge in API-aware code generation: \textbf{LLMs often default to historical coding patterns rather than leveraging modern APIs, even when the newer APIs were available before their knowledge cutoff.} This issue arises due to multiple factors:  
\begin{itemize}
    \item Gradual API Adoption. Even after stabilization, new APIs may take time to be widely adopted, leading to training data being dominated by older patterns.
    \item Persistence of Legacy Idioms. Common programming practices persist in the ecosystem long after better alternatives become available. 
    \item Training Data Bias. Without explicit version-specific guidance, LLMs tend to favor patterns they encountered more frequently, potentially overlooking API improvements.  
\end{itemize}

This challenge underscores the necessity of a dedicated benchmark to assess LLMs' ability to adapt to API evolution in real-world coding scenarios. \textbf{Existing code generation benchmarks often fail to systematically evaluate whether models can utilize the latest API features, that API evolution knowledge, instead measuring performance on static datasets that do not reflect ongoing language and ecosystem changes.} A static benchmark is insufficient for evaluating API-aware code generation, as it cannot account for the continuous evolution of programming languages, libraries, and best practices.  

To address this limitation, \textbf{our benchmark is designed to evolve alongside API changes, ensuring that evaluation remains relevant as new APIs are introduced and old patterns become obsolete.} Rather than relying on manually curated tasks, our dataset construction process is designed to be \textbf{automated}, dynamically incorporating API updates to create new evaluation instances. This automation enables continuous and scalable assessment of LLMs' ability to generate optimal, up-to-date code.  

In summary, our work fills a critical gap in current benchmarks by providing a systematic and dynamically evolving evaluation framework. By focusing on API evolution awareness, we enable a more realistic assessment of LLMs’ capabilities, ensuring that they not only generate functionally correct code but also adapt to the best available practices in a given Rust version.



%These challenges underscore the necessity of developing benchmarks specifically  Even when models theoretically "know" about an API due to their knowledge cutoff dates, they may still generate suboptimal code that reflects historical patterns rather than current optimal approaches. This motivates our approach: a dataset specifically designed to evaluate whether models can generate optimal code that leverages the best available APIs for a specific Rust version, rather than defaulting to potentially outdated patterns that may be overrepresented in their training data.


% Figure \ref{fig:motivation} presents a programming task that implicitly requires using this newly stabilized API. When presented with this task, \claude~\cite{xx}, a state-of-the-art (SOTA) LLM with a knowledge cutoff prior to Rust 1.82.0, generates code that relies on the older, less efficient pattern using \texttt{MaybeUninit::uninit()} followed by \texttt{Box::new()}. While this approach is functional, it incurs unnecessary initialization overhead and misses the opportunity for improved performance. However, when the same model is augmented API evaluation information, it correctly utilizes the newly stabilized \texttt{Box::new\_uninit()} API, resulting in more efficient code.

% The example shows that even the LLMs

% This example illustrates three key challenges in API-aware code generation: (1) LLMs have limited awareness of recently evolved APIs due to their knowledge cutoff dates, (2) generating optimal code often requires understanding subtle API transitions that may not alter functionality but significantly impact performance or safety, and (3) without explicit version-specific guidance, LLMs default to patterns they were trained on, potentially missing API improvements.

% Moreover, neither traditional documentation approaches nor existing code generation methods adequately address this problem. Standard API documentation typically describes current functionality without capturing the evolution history, while existing benchmarks for code generation lack version-specific evaluation capabilities. This motivates our approach: a extensive dataset that captures API evolution patterns and enables evaluation of how effectively models adapt to API changes over time.

% These challenges underscore the necessity of developing benchmarks specifically designed to assess the ability of LLMs to understand and generate code that incorporates API evolution. As the evolution of APIs continues rapidly, and considering that large models are also frequently updated, it is crucial to have an evaluation framework that continuously reflects the models' capabilities in adapting to these changes. To achieve this, an automated approach to dataset construction is imperative. Such an approach will ensure that the dataset remains relevant and accurately reflects the evolving nature of APIs, enabling consistent and up-to-date evaluations of model performance in real-world scenarios.

% By focusing on API evolution, our work aims to fill a critical gap in the current benchmarks, providing a comprehensive and dynamic evaluation of large models' understanding and generation abilities, while also supporting continuous updates in response to ongoing API changes.



==> sections/X_move_to_2__MotivationExample.tex <==
\section{Motivation Example}
\label{sec:motivation}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/2_Motivation/motivation.pdf}
    \caption{Motivation Example}
    \label{fig:motivation}
\end{figure}

To illustrate the challenges of code generation in the context of evolving APIs, we consider a real-world case from the Rust ecosystem. In Rust 1.77.0 (released in March 2024), the \texttt{slice::first\_chunk\_mut} method\footnote{XXX} was stabilized, providing a safer and more efficient way to obtain a reference to the first N elements of a slice as a fixed-size array.  
Figure \ref{fig:motivation} presents a programming task that implicitly requires using an API that was stabilized well before the model’s knowledge cutoff date. However, when prompted with this task, \claude~\cite{anthropic2024claude3}—a state-of-the-art (SOTA) LLM with a knowledge cutoff in April 2024—still generates code relying on an older, less safe pattern involving unsafe pointer casting and manual length checking. While this approach remains functional, it introduces unnecessary unsafe code and forgoes the benefits of improved safety and readability. In contrast, when explicitly informed about the API evolution, the same model correctly utilizes \texttt{slice::first\_chunk\_mut}, producing more concise and robust code.  

This example highlights a fundamental challenge in API-aware code generation: \textbf{LLMs often default to historical coding patterns rather than leveraging modern APIs, even when the newer APIs were available before their knowledge cutoff.} This issue arises due to multiple factors:  
\begin{itemize}
    \item Gradual API Adoption. Even after stabilization, new APIs may take time to be widely adopted, leading to training data being dominated by older patterns.
    \item Persistence of Legacy Idioms. Common programming practices persist in the ecosystem long after better alternatives become available. 
    \item Training Data Bias. Without explicit version-specific guidance, LLMs tend to favor patterns they encountered more frequently, potentially overlooking API improvements.  
\end{itemize}

This challenge underscores the necessity of a dedicated benchmark to assess LLMs' ability to adapt to API evolution in real-world coding scenarios. \textbf{Existing code generation benchmarks often fail to systematically evaluate whether models can utilize the latest API features, that API evolution knowledge, instead measuring performance on static datasets that do not reflect ongoing language and ecosystem changes.} A static benchmark is insufficient for evaluating API-aware code generation, as it cannot account for the continuous evolution of programming languages, libraries, and best practices.  

To address this limitation, \textbf{our benchmark is designed to evolve alongside API changes, ensuring that evaluation remains relevant as new APIs are introduced and old patterns become obsolete.} Rather than relying on manually curated tasks, our dataset construction process is designed to be \textbf{automated}, dynamically incorporating API updates to create new evaluation instances. This automation enables continuous and scalable assessment of LLMs' ability to generate optimal, up-to-date code.  

In summary, our work fills a critical gap in current benchmarks by providing a systematic and dynamically evolving evaluation framework. By focusing on API evolution awareness, we enable a more realistic assessment of LLMs’ capabilities, ensuring that they not only generate functionally correct code but also adapt to the best available practices in a given Rust version.



%These challenges underscore the necessity of developing benchmarks specifically  Even when models theoretically "know" about an API due to their knowledge cutoff dates, they may still generate suboptimal code that reflects historical patterns rather than current optimal approaches. This motivates our approach: a dataset specifically designed to evaluate whether models can generate optimal code that leverages the best available APIs for a specific Rust version, rather than defaulting to potentially outdated patterns that may be overrepresented in their training data.


% Figure \ref{fig:motivation} presents a programming task that implicitly requires using this newly stabilized API. When presented with this task, \claude~\cite{xx}, a state-of-the-art (SOTA) LLM with a knowledge cutoff prior to Rust 1.82.0, generates code that relies on the older, less efficient pattern using \texttt{MaybeUninit::uninit()} followed by \texttt{Box::new()}. While this approach is functional, it incurs unnecessary initialization overhead and misses the opportunity for improved performance. However, when the same model is augmented API evaluation information, it correctly utilizes the newly stabilized \texttt{Box::new\_uninit()} API, resulting in more efficient code.

% The example shows that even the LLMs

% This example illustrates three key challenges in API-aware code generation: (1) LLMs have limited awareness of recently evolved APIs due to their knowledge cutoff dates, (2) generating optimal code often requires understanding subtle API transitions that may not alter functionality but significantly impact performance or safety, and (3) without explicit version-specific guidance, LLMs default to patterns they were trained on, potentially missing API improvements.

% Moreover, neither traditional documentation approaches nor existing code generation methods adequately address this problem. Standard API documentation typically describes current functionality without capturing the evolution history, while existing benchmarks for code generation lack version-specific evaluation capabilities. This motivates our approach: a extensive dataset that captures API evolution patterns and enables evaluation of how effectively models adapt to API changes over time.

% These challenges underscore the necessity of developing benchmarks specifically designed to assess the ability of LLMs to understand and generate code that incorporates API evolution. As the evolution of APIs continues rapidly, and considering that large models are also frequently updated, it is crucial to have an evaluation framework that continuously reflects the models' capabilities in adapting to these changes. To achieve this, an automated approach to dataset construction is imperative. Such an approach will ensure that the dataset remains relevant and accurately reflects the evolving nature of APIs, enabling consistent and up-to-date evaluations of model performance in real-world scenarios.

% By focusing on API evolution, our work aims to fill a critical gap in the current benchmarks, providing a comprehensive and dynamic evaluation of large models' understanding and generation abilities, while also supporting continuous updates in response to ongoing API changes.


